Support recovery and sup-norm convergence rates for sparse pivotal estimation

In high dimensional sparse regression, pivotal estimators are estimators for which the optimal regularization parameter is independent of the noise level. The canonical pivotal estimator is the square-root Lasso, formulated along with its derivatives as a "non-smooth + non-smooth" optimization problem. Modern techniques to solve these include smoothing the datafitting term, to benefit from fast efficient proximal algorithms. In this work we show minimax sup-norm convergence rates for non smoothed and smoothed, single task and multitask square-root Lasso-type estimators. Thanks to our theoretical analysis, we provide some guidelines on how to set the smoothing hyperparameter, and illustrate on synthetic data the interest of such guidelines.

==> sections/5_calibrate_multivariate_regression.tex <==
% TEX root = ../bounds.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Calibrate Multivariate Regression \citet{Liu_Wang_Zhao15}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mm{discuss what we do with this one. Smooth it too?}
We consider the Calibrate Multivariate Regression \citet{Liu_Wang_Zhao15} with an $\ell_{2,1}$ penalty defined as the following:
%
\begin{problem}\label{pb:calibrate_multivar_sqrt}
      \argmin_{\Beta \in \bbR^{p\times q}}
      \frac{1}{n q} \normin{(Y - X \Beta)^\top}_{2, 1}
      + \lambda \norm{\Beta}_{2,1}
      \enspace .
\end{problem}
%
Assuming that $\hat \Epsilon_{:, t} \neq 0$, then with $\hat z_j \in \partial \norm{\cdot}_2 (\hat \Beta_{j, :}) $ the KKT reads:
\begin{equation}
    \frac{1}{n q} \hat \Epsilon
    = \lambda \diag \left ( \hat z_j \right ) \hat \Beta \diag \left (\normin{\hat \Epsilon_{:, t}}_2 \right) \enspace .
\end{equation}
%
This leads to
\begin{equation}
    \frac{1}{n q} \normin{\hat \Epsilon}_{2, \infty}
    \leq \lambda \max_{t}\normin{\hat \Epsilon_{:, t}}_2  \enspace .
\end{equation}
%
\begin{align}
    \tfrac{1}{q} \normin{\Psi \Delta}_{2, \infty}
     &= \tfrac{1}{nq}\normin{X^\top (X \hat \Beta - Y + \Epsilon )}_{2, \infty} \nonumber\\
    %
    & \leq
    \tfrac{1}{nq} \normin{X^\top \hat \Epsilon}_{2, \infty}
    + \tfrac{1}{nq} \normin{X^\top \Epsilon}_{2, \infty}  \nonumber\\
    %
    & \leq
    \tfrac{1}{nq} \max_{t}\normin{\hat \Epsilon_{:, t}}_2
    + \tfrac{1}{nq}\normin{X^\top \Epsilon}_{2, \infty} \nonumber
  \end{align}
%


==> sections/app_lasso.tex <==
%!TEX root = ../bounds.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Bounds for the Lasso}
\label{sec:bounds_for_the_lasso}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Throughout the paper we will need to use some Fenchel transforms, recalled in \Cref{tab:fenchel_transforms}.
The reader should be aware that we use ${}^*$ to denote the true value of the parameters (\ie, $\beta^*$), but when applied to \emph{functions}, it refers to the Fenchel transform.
\begin{table}
  \centering
  \caption{Useful Fenchel transforms}
  \label{tab:fenchel_transforms}
  \newcommand*{\SetEqNum}{%
    \refstepcounter{equation}%
    \thetag\theequation
  }
  \newcommand*{\DisplayEq}[1]{%
    \ensuremath{\displaystyle #1}%
  }
  \begin{tabular}{ccr}
    \toprule
    Function &  Fenchel transform
    \\ \midrule
    $h^*$
    & \DisplayEq{h , \quad \forall h \in \Gamma_0(\bbR^d)}
    & \SetEqNum\label{eq:fenchel-involution}
    \\
    \addlinespace
    $g \infconv h$
    & \DisplayEq{g^* + h^*}
    & \SetEqNum\label{eq:inf-conv-morphism}
    \\
    \addlinespace
    $a h \left(\frac{\cdot}{a}\right)$
    & \DisplayEq{a h^*, \quad \forall a > 0}
    & \SetEqNum\label{eq:inf-conv-scaling}
    \\
    \addlinespace
    $\norm{\cdot}_{p}$
    & \DisplayEq{\iota_{\cB_{p^*}} , \text{ where } \tfrac {1}{p} + \tfrac{1}{p^*} = 1}
    & \SetEqNum\label{eq:fenchel-norm}
    \\
    \addlinespace
    $(h+\delta)$
    & \DisplayEq{h^*-\delta, \quad \forall \delta \in \bbR}
    & \SetEqNum\label{eq:fenchel-translation}
    \\
    \addlinespace
    $\tfrac{1}{2} \norm{\cdot}^2$
    & \DisplayEq{\tfrac{1}{2} \norm{\cdot}^2}
    & \SetEqNum\label{eq:fenchel-norm2}
    \\ \bottomrule
  \end{tabular}
\end{table}

\begin{definition}[Lasso, \citet{Tibshirani96}] The Lasso estimator is
  defined as the solution\footnote{Following \citet{vandeGeer16} we do not express in our notation that the Lasso may not generate a unique solution.
        In this section $\betahat$ will be \emph{a solution} of the Lasso.} of the optimization problem
    \begin{problem}\label{pb:lasso}
        \betahat
        \eqdef
        \argmin_{\beta \in \bbR^p}
        \frac{1}{2n} \norm{y - X \beta}_2^2 + \lambda \norm{\beta}_1
        \enspace .
    \end{problem}
\end{definition}
%
The main result of this section, proved in \citet[Thm 1 p. 93]{Lounici08}, is a bound in estimation on the regression coefficients when the noise level $\sigma$ is known.

\begin{restatable}[Estimation control]{theorem}{restatelassosupnorm}
\label{thm:lasso_sup_norm}
% \begin{theorem}\label{thm:lasso_sup_norm}
    Take $\lambda = A \sigma \sqrt{(\log p) / n}$ and $A > 2 \sqrt{2}$.
    %
    Let \Cref{assum:gauss_noise,assum:mut_inco} be satisfied, then
    \begin{align}
    \bbP\left(
        \normin{\betahat-\betastar}_\infty  \leq c_2 \lambda
    \right)
    \geq 1-p^{1-A^{2} / 8} \enspace,
     \end{align}
     with
     $c_2 = \frac{3}{2}
        \left
            ( 1 + \frac{16}{7(\alpha-1)}
        \right )$, and $\alpha$ satisfying \Cref{assum:mut_inco}.
% \end{theorem}
\end{restatable}

The proof of \Cref{thm:lasso_sup_norm} needs preliminary lemmas detailed in following sections.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{KKT conditions}
\label{sub:lasso_kkt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

First we prove that the Lasso estimator satisfies the \emph{Dantzig constraint}:
%
\begin{align} \label{eq:dantzig_constraint}
    \frac{1}{n} \norm{X^{\top}(y-X \betahat)}_\infty
    \leq \lambda \enspace .
\end{align}
%
This is trivial to check by using the KKT conditions for \Cref{pb:lasso}:
\begin{align}
    \begin{cases}
            \frac{1}{n} X_{j}^\top (y-X \betahat)
            = \lambda \sign \betahat_{j} \quad ,
            & \text { if } \betahat_{j} \neq 0 \enspace,  \\
        % %
            \frac{1}{n} |X_{j}^{\top}(y-X \betahat)|
            \leq
            \lambda \quad ,
            & \text { if } \betahat_{j} = 0
            \enspace .
        \end{cases}
        %
\end{align}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bounds in prediction}
\label{sub:bounds_in_prediction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Let us define $\hat \varepsilon \eqdef y - X \hat\beta$ and consider the event $\cA$:
\begin{equation} \label{eq:event_lso}
  \cA \eqdef \left \{ \frac{1}{n}  \norm{X^{\top} \varepsilon }_\infty
  \leq
  \frac{\lambda}{2}  \right \} \enspace .
\end{equation}
%
\begin{lemma}\label{lem:lso_bds_pred}
  Let  \Cref{assum:gauss_noise,assum:mut_inco} be satisfied.
  Then with $\Delta = \betahat - \betastar$, on $\cA$:
  \begin{lemmaenum}
      \item $ \tfrac1n \normin{X^\top(X\betastar - X\betahat)}_\infty
            \leq
            \frac{3 \lambda}{2} \enspace ,$ \label{lem:lso_bds_pred_a}
      \item $\norm{\Delta_{S^{* c}}}_{1}
            \leq  3 \norm{\Delta_{S^*}}_{1} \enspace .$  \label{lem:lso_bds_pred_b}
  \end{lemmaenum}
\end{lemma}
%
\begin{proof}
%
Proof of \Cref{lem:lso_bds_pred_a} combines the Dantzig constraint \eqref{eq:dantzig_constraint} and the event $\cA$:
\begin{align}
    \frac 1n \normin{X^\top (X\betastar - X\betahat)}_\infty
    &= \frac 1n \normin{X^\top (y - X\betahat + \varepsilon)}_\infty \nonumber \\
    &\leq  \frac 1n \normin{X^\top \hat \varepsilon}_\infty + \frac 1n \normin{X^\top \varepsilon}_\infty \nonumber \\
    &\leq  \lambda + \frac 1n \normin{X^\top \varepsilon}_\infty & \text{ (using \Cref{eq:dantzig_constraint})} \nonumber \\
    & \leq \lambda  + \frac{\lambda}{2} & \text{ (using \Cref{eq:event_lso})} \nonumber\\
    & \leq  \frac{3}{2} \lambda \nonumber \enspace .
\end{align}
%
For \Cref{lem:lso_bds_pred_b}: The Lasso estimator is based on an optimization problem like \Cref{pb:generic_optim_pb} with $f = \frac{1}{2n} \normin{\cdot}^2$, which is convex and satisfies $\partial{f}(z) = \{ \frac{z}{n} \}$.
Therefore, on $\cA$:
\begin{equation}
  \frac{1}{n}  \norm{X^{\top} \varepsilon }_\infty
  \leq
  \frac{\lambda}{2} \enspace, \text{ with } \frac{\varepsilon}{n} \in \partial{f}(\varepsilon) \enspace .
\end{equation}
We can thus apply \Cref{lem:bds_S_c_S} with $c_3 = \frac{1}{2}$, leading to \Cref{lem:lso_bds_pred_b}.
%   %
%   \begin{align}
%       \frac{1}{n} \normin{y-X \betahat}_{2}^{2}
%       + 2 \lambda \normin{\betahat}_{1}
%         &\leq \frac{1}{n}\norm{\varepsilon}_{2}^{2}+2 \lambda \norm{\betastar}_{1}\\
%       %
%       2 \lambda \normin{\betahat}_1
%         &\leq 2 \lambda \normin{\betastar}_1
%       + \frac{2}{n} (\betahat-\betastar)^{\top} X^{\top} \varepsilon \enspace .
%   \end{align}
%   %
%   H\"older inequality and Gaussian tail inequality~\eqref{eq:gauss_tail} lead to
%   \begin{align}
%       2 \normin{\betahat}_1
%       &\leq
%         2 \norm{\betastar}_1 + \normin{\betahat - \betastar}_1 \\
%       2 \normin{\betahat}_1 + \normin{\betahat - \betastar}_1
%       &\leq
%        2 \left (
%           \normin{\betastar}_1
%           + \normin{\betahat - \betastar}_1
%           \right) \enspace ,\\
%       %
%       \normin{\betahat - \betastar}_1
%       %
%       &\leq 2 \left (
%           \normin{\betahat - \betastar}_1
%           + \normin{\betastar}_1
%           - \normin{\betahat}_1
%           \right) \enspace .
%   \end{align}
%   Let us remark that $\absin{\betahat_j - \betastar_j}
%   + \absin{\beta^*_j}
%   - \absin{\betahat_j} = 0$ if $j \notin S^*$, leading to
%   \begin{align}
%           \normin{\betahat - \betastar}_1
%           + \norm{\betastar}_1
%           - \normin{\betahat}_1
%           =
%           \norm{\Delta_{S^*}}_1
%           + \norm{\betastar_{S^*}}_1
%           - \normin{\betahat_{S^*}}_1
%           \leq
%           2 \norm{\Delta_{S^*}}_1 \enspace .
%   \end{align}
% %
% Combining the last two inequalities leads to
% %
%   \begin{align}
%       \norm{\Delta}_1
%       %
%       & \leq 4 \norm{\Delta_{S^*}}_1  \enspace,\\
%       %
%       \norm{\Delta_{S^{*c}}}_1
%       %
%       & \leq 3 \norm{\Delta_{S^*}}_1 \enspace .
%   \end{align}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Control  of the event}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{lemma}\label{lem:control_event_lasso}
  Take $\lambda = A \sigma \sqrt{(\log p) / n}$ and $A > 2 \sqrt{2}$, then:
  \begin{equation}
    \bbP(\cA) \geq 1 - p^{\frac{A^2}{8}} \enspace .
  \end{equation}
\end{lemma}
%
\begin{proof}
  Let us define $Z \eqdef \tfrac{1}{n} X^{\top} \varepsilon$ ; then we can express $\cA$ as:
  \begin{align}
      \cA = \bigcap_{j=1}^{p}\left\{\left|Z_{j}\right| \leq \lambda / 2\right\} \enspace .
   \end{align}
  %
  Standard Gaussian tail inequalities hold: since $\normin{X_j} = \sqrt{n}$, $Z_j \sim \cN(0, n \sigma^2)$ and
  \begin{align}
      \bbP\left(\cA^c\right)
      %
      & \leq p \, \bbP \left(\left|Z_{1}\right| \geq \lambda / 2\right) \nonumber \\
      %
      & \leq p \exp \left(-\frac{n}{2 \sigma^{2}}\left(\frac{\lambda}{2}\right)^{2}\right) \nonumber \\
      %
      & \leq p^{1-\frac{A^{2}}{8}} \enspace.
  \end{align}
\end{proof}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bounds in estimation}
\label{sub:bounds_in_estimation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section we prove \Cref{thm:lasso_sup_norm}, which we first recall:
\restatelassosupnorm*
%
\begin{proof}(\Cref{thm:lasso_sup_norm})
    Let us warn the reader that in the following proof the results are considered on the event $\cA$.
    Let $\Psi$ and $\alpha$ satisfy \Cref{assum:mut_inco}, \Cref{lem:bnd_l_infty_l_infty,lem:lso_bds_pred_b} \mm{wrong order I don't know why} lead to:
    \begin{align}
      \normin{\Delta}_\infty
      & \leq \left(
          1 + \frac{16}{7(\alpha - 1) } \right) \norm{\Psi \Delta}_\infty \nonumber \\
      & \leq \frac{3}{2}\left(
          1 + \frac{16}{7(\alpha - 1) } \right) \lambda & \text{(using \Cref{lem:lso_bds_pred_a}).} \enspace.
    \end{align}
  Combined with \Cref{lem:control_event_lasso} this leads to the desired result.
\end{proof}


==> sections/app_smoothconco.tex <==
%TEX root=bounds.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Smoothed concomitant Lasso}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{definition}[Smoothed Concomitant Lasso]
  For $\lambda > 0$ and $\sigmamin > 0$, the smoothed concomitant Lasso coefficients and noise level estimators are obtained as:
  \begin{problem}\label{pb:smoothconco}
    (\hat\beta, \hat\sigma) =
      \argmin_{\beta, \sigma \geq \sigmamin}
      \frac{1}{2n \sigma} \normin{y - X\beta}^2 + \frac{\sigma}{2}
      + \lambda \normin{\beta}_1 \enspace .
   \end{problem}
\end{definition}
%
Let us recall that $\betahat$ is also the solution of the following optimization problem:
\begin{problem}\label{pb:link_smoothconco_sqrtlasso}
  \hat\beta = \argmin_{\beta}
      \left(  \normin{\cdot} \infconv \omega_{\sigmamin} \right)
      \left( \frac{1}{\sqrt{n}}(y - X\beta) \right)
    + \lambda \normin{\beta}_1
    \enspace ,
 \end{problem}
 with $\omega_{\sigmamin} \eqdef \frac{\sigmamin}{2} \norm{\cdot}^2 + \frac{1}{2} \sigmamin$.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Recall on smoothing}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
We will use some properties of inf-convolution smoothing with $\omega_{\sigmamin}$.
In all this section, the variable is a matrix $Z \in \bbR^{n \times q}$.
\begin{lemma}\label{lemma:conco_p_q}
Let\footnote{there is a notation overloading here as $p$ referred to the number of features. It is clear from the context that in this section, a different $p$ is used as the order of the Schatten norm.} $c \in \bbR, p \in [1, \infty]$. Let $p^* \in [1, \infty]$ be the H\"{o}lder conjugate of $p$: $\frac{1}{p} + \frac{1}{p^*} = 1$. For the choice $\omega(\cdot) = \frac{1}{2}\norm{\cdot}^2 + c$,  the following holds true:
    \begin{align}
        \left(\norm{\cdot}_{\mathscr{S}, p} \infconv \omega_{\sigmamin}\right)(Z)
        &= \frac{1}{2\sigmamin}\norm{Z}_F^2
          + c \sigmamin
          - \frac{\sigmamin}{2} \norm{\Pi_{\cB_{\mathscr{S}, p^*}}\left(\tfrac{Z}{\sigmamin}\right) -\tfrac{Z}{\sigmamin}}_F^2 \enspace.
    \end{align}
\end{lemma}
%
\begin{proof}
  \begin{align}
    \left(\norm{\cdot}_{\mathscr{S}, p} \infconv \omega_{\sigmamin} \right)(Z)
    % & = \left(\norm{\cdot}_{\mathscr{S}, p} \infconv \omega_{\sigmamin}\right)^{**}(Z) & \text{(using \cref{eq:fenchel-involution})}  \nonumber\\
    %
    & = \left(\norm{\cdot}_{\mathscr{S}, p}^* + \omega_{\sigmamin}^*\right)^{*}(Z)
      & \text{(using \cref{eq:fenchel-involution,eq:inf-conv-morphism})}\nonumber  \\
      %
    & = \left(\iota_{\cB_{\mathscr{S}, p^*}}
      + \tfrac{\sigmamin}{2} \norm{\cdot}_F^2
      - c \sigmamin \right)^*(Z) \nonumber
      &\text{(using \cref{eq:fenchel-norm} and $\omega_{\sigmamin}^* = \tfrac{\sigmamin}{2} \normin{\cdot}_F^2
      - c \sigmamin $)} \\
      %
    & = \left(\tfrac{\sigmamin}{2} \norm{\cdot}_F^2
      + \iota_{\cB_{\mathscr{S}, p^*}}\right)^*(Z)
      + c \sigmamin
      & \text{(using \cref{eq:fenchel-translation})}\enspace. \label{eq:first_lp_case}
  \end{align}
  Now, by definition,\mm{what is $c$ and sure about the sigmamin on top?}
  \begin{align}
      \left(\frac{\sigmamin}{2} \normin{\cdot}_F^2 + \iota_{\cB_{\mathscr{S},p^*}}\right)^*(Z)
      %
      &= \sup_{U \in \bbR^{n \times q}} \left( \langle U, Z \rangle - \frac{\sigmamin}{2} \normin{U}_F^2 - \iota_{\cB_{\mathscr{S},p^*}}(U) \right) \nonumber \\
      %
      &= \sup_{U \in \cB_{\mathscr{S}, p^*} } \left(\langle U, Z \rangle - \frac{\sigmamin}{2} \normin{U}_F^2 \right)\nonumber \\
      &= - \sigmamin \cdot \inf_{U \in \cB_{\mathscr{S}, p^*} } \left(\tfrac{1}{2} \normin{U}_F^2 - \left\langle U, \tfrac{Z}{\sigmamin} \right\rangle \right)\nonumber \\
      %
      &= - \sigmamin \cdot \inf_{U \in \cB_{\mathscr{S}, p^*} } \left(\tfrac{1}{2} \norm{U -\tfrac{Z}{\sigmamin}}_F^2 - \tfrac{1}{2\sigmamin^2}\norm{Z}_F^2\right)  \nonumber \\
      &= \tfrac{1}{2\sigmamin}\norm{Z}_F^2 - \tfrac{\sigmamin}{2}  \cdot \inf_{U \in \cB_{\mathscr{S}, p^*} } \left(\norm{U -\tfrac{Z}{\sigmamin}}_F^2
      \right) \nonumber \\
      &= \tfrac{1}{2\sigmamin}\norm{Z}_F^2 -
          \tfrac{\sigmamin}{2}  \norm{\Pi_{\cB_{\mathscr{S}, p^*}}\left(\tfrac{Z}{\sigmamin}\right) -\tfrac{Z}{\sigmamin}}_F^2
      \label{eq:in_proof_projection_lq} \enspace.
  \end{align}\mm{cleaner and shorter if we use inf convolution result?}
The result follows by combining \cref{eq:first_lp_case,eq:in_proof_projection_lq}.
%
\end{proof}
%
\begin{lemma} For any $\sigmamin > 0$ and $Z$ in $\bbR^{n \times q}$, we have:
  \begin{lemmaenum}
    \item \label{lem:link_infconv_conco} $\left(\norm{\cdot}_{F} \infconv \omega_{\sigmamin}\right)(Z)
    = \min_{\sigma \geq \sigmamin} \left(\tfrac{1}{2 \sigma} \norm{Z}_F^2 + \tfrac{\sigma}{2}\right) \enspace ,$
    \item \label{lem:infconv_greater} $\normin{\cdot}_F \infconv \omega_{\sigmamin} (Z) \geq \normin{Z}_F \enspace.$
    % \mathurin{oops}
    % \item \label{lem:smoothing_threshold} $\normin{\cdot}_2 \geq \sigmamin \implies \normin{\cdot}_2 \infconv \omega_{\sigmamin} (x) = \normin{x}_2 \enspace .$
  \end{lemmaenum}
\end{lemma}
%
\begin{proof}
  We apply \Cref{lemma:conco_p_q} with $c=\frac{1}{2}$, $p = p^* = 2$.
  \begin{equation}
    \Pi_{\cB_{F}} \left ( \frac{Z}{\sigmamin}\right ) =
    \begin{cases}
       0  \enspace, &\text{if $\normin{\frac{Z}{\sigmamin}}_F \leq 1 $} \enspace, \\
       \frac{Z}{\normin{Z}_F} \enspace, & \text{else} \enspace,
    \end{cases} \nonumber
  \end{equation}
which leads to:
  \begin{equation}
    \left(\norm{\cdot}_{F} \infconv \omega_{\sigmamin}\right)(Z) =
    \begin{cases}
      \frac{1}{2\sigmamin}\norm{Z}_F^2
      + \frac{1}{2} \sigmamin \enspace, &\text{if $\normin{Z}_F \leq  \sigmamin$}\\
      \normin{Z}_F \enspace, & \text{else} \enspace ,
    \end{cases} \label{eq:huber_formula_conco}
  \end{equation}
  which easily proves \Cref{lem:link_infconv_conco,lem:infconv_greater}:
  % \begin{equation}
    % \left(\norm{\cdot}_{F} \infconv \omega_{\sigmamin}\right)(Z) \geq \norm{Z}_{F} \enspace .
  % \end{equation}
  % Moreover \Cref{eq:huber_formula_conco} also leads to \Cref{lem:link_infconv_conco}:
  % \begin{equation}
  %   \left(\norm{\cdot}_{F} \infconv \omega_{\sigmamin}\right)(Z)
  %   = \min_{\sigma \geq \sigmamin} \left(\tfrac{1}{2 \sigma} \norm{Z}_F^2 + \tfrac{\sigma}{2}\right) \enspace .
  % \end{equation}
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{KKT}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\Cref{pb:link_smoothconco_sqrtlasso} is an instance of \Cref{pb:generic_optim_pb} with
$f = (\normin{\cdot} \infconv \omega_{\sigmamin})(\frac{\cdot}{\sqrt{n}})$.
We have $f^* = (\normin{\cdot}^* + \omega_{\sigmamin}^*)(\sqrt{n} \cdot)$
and therefore a dual formulation of \Cref{pb:smoothconco} is:\mm{add conjugate of smoothing kernel in table?}
\begin{problem}
  \thetahat \in \argmax \lambda\theta^\top y + \frac{\sigmamin}{2}(1 - n \lambda^2 \normin{\theta}^2)  \quad \st \quad \normin{X^\top \theta}_\infty \leq 1 \; \text{and} \; \normin{\theta} \leq 1 / \lambda \sqrt{n} \enspace.
\end{problem}
% A Lagrangian for \Cref{pb:smoothconco} is
% \begin{equation}
%   \cL(\beta, z, \sigma, \theta, \nu) =
%   \frac{1}{2n \sigma} \normin{z} ^2 + \frac{n \sigma}{2}
%   + \lambda \normin{\beta}_1 + \theta^\top(z - y + X\beta) + \nu (\sigmamin - \sigma) \enspace.
% \end{equation}
%
The optimality conditions read:
\begin{equation}
  \begin{cases}
    \hat z = y - X \hat \beta \enspace, \\
    - X^\top \hat \theta / \lambda \in \partial \normin{\cdot}_1(\hat \beta) \enspace , \\
    \hat \theta = y - X \betahat \enspace , \\
    \sigma = \max (\sigmamin, {\normin{y - X \hat \beta}} / {\sqrt{n}}) \enspace.
  \end{cases}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Dantzig constraint}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let us recall that $\hat \varepsilon \eqdef y - X \hat \beta$.
%
\begin{lemma}
  Let $\eta, \sigma_0$ satisfy \Cref{assum:high_noise}, let $\sigmamin \leq \sigma_0$, then on event:
  \begin{equation} \label{eq:event_1_smoothed_sqrtlso}
    \left\{ \frac{\normin{\varepsilon}_2}{\sqrt{n}} \geq \sigma_0 \right\} \enspace,
  \end{equation}
  \begin{equation}
    \frac{\normin{\hat \varepsilon}_2}{\sqrt{n}}
     \leq
     (1 + \eta) \frac{\normin{\varepsilon}_2}{\sqrt{n}} \enspace
  \end{equation}
\end{lemma}
%
\begin{proof}
  The proof comes from the minimality of $\hat \beta$, on $\left\{ \frac{\normin{\varepsilon}_2}{\sqrt{n}} \geq \sigma_0 \right\}$:
  \begin{align}
    \left(  \normin{\cdot}_2 \infconv \omega_{\sigmamin} \right)
    \left( \frac{1}{\sqrt{n}}\hat \varepsilon \right)
    + \lambda \normin{\hat \beta}_1
    &\leq
      \left(  \normin{\cdot}_2 \infconv \omega_{\sigmamin} \right)
      \left( \frac{1}{\sqrt{n}} \varepsilon\right)
      + \lambda \normin{\beta^*}_1 \nonumber \\
    \left(  \normin{\cdot}_2 \infconv \omega_{\sigmamin} \right)
    \left( \frac{1}{\sqrt{n}} \hat \varepsilon \right)
    &\leq
      \left(  \normin{\cdot}_2 \infconv \omega_{\sigmamin} \right)
      \left( \frac{1}{\sqrt{n}} \varepsilon \right)
      + \lambda \normin{\beta^*}_1 & \text{(since $\normin{\hat \beta}_1\geq 0$)} \nonumber \\
    \frac{1}{\sqrt{n}} \normin{\hat \varepsilon}_2
    &\leq
      \left(  \normin{\cdot}_2 \infconv \omega_{\sigmamin} \right)
      \left( \frac{1}{\sqrt{n}} \varepsilon \right)
      + \lambda \normin{\beta^*}_1 & \text{(\Cref{lem:infconv_greater})}\nonumber \\
   &\leq  \frac{1}{\sqrt{n}} \normin{\varepsilon}_2
    + \lambda \normin{\beta^*}_1 &\text{(\Cref{lem:link_infconv_conco,eq:event_1_smoothed_sqrtlso})}\nonumber \\
    &\leq  (1 + \eta ) \frac{1}{\sqrt{n}} \normin{\varepsilon}_2 & \text{(\Cref{assum:high_noise})} \label{eq:approx_epsilon_smoothed_sqrtlso} \enspace .
  \end{align}
\end{proof}
%
As before\mm{be more precise} it can be shown from the KKT conditions that the Smoothed Concomitant Lasso verifies a generalized Dantzig constraint \mm{on the event that we must name}:
%
\begin{align}\label{eq:dantzig_constr_ssqrtl_sigmahat}
  \frac{1}{n} \norm{ X^{\top} (y - X \betahat)}_\infty
  &\leq
  \lambda \max \left( \frac{\norm{ \hat \varepsilon}_2}{\sqrt{n}}, \sigmamin \right) & \text{(KKT)} \nonumber\\
  &\leq \lambda \max \left( (1 + \eta) \frac{\normin{\varepsilon}_2}{\sqrt{n}}, \sigmamin  \right) & \text{(using \Cref{eq:approx_epsilon_smoothed_sqrtlso})} \nonumber \\
  & \leq \lambda (1 + \eta) \frac{\normin{\varepsilon}_2}{\sqrt{n}} & \text{(using \Cref{eq:event_1_smoothed_sqrtlso})}
  \enspace .
\end{align}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bounds in prediction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mm{TODO check that this is not included in tex}
\begin{lemma}\label{lem:smth_sqrtlasso_bds_pred}
  Let \Cref{assum:gauss_noise,assum:mut_inco} be satisfied.
  Then with $\Delta = \betahat - \betastar$ and $c_0=\frac{2}{\eta} - 1$, on $\cA_1$:
  \begin{lemmaenum}
      \item
          $\tfrac1n \normin{X^\top(X\betastar - X\betahat)}_\infty
          \leq
          2 \lambda \sigmamax \enspace ,$ \label{lem:smth_sqrt_lso_bds_pred_a}
      \item $\norm{\Delta_{S^{* c}}}_{1}
            \leq
            c_0 \norm{\Delta_{S^*}}_{1} \enspace .$  \label{lem:smth_sqrt_lso_bds_pred_b}
  \end{lemmaenum}
\end{lemma}
%
\begin{proof}
   As before the proof of \Cref{lem:smth_sqrt_lso_bds_pred_a} comes from the KKT and the concentration on $\cA_1$:
  \begin{align}
    \tfrac1n \normin{X^\top(X\betastar - X\betahat)}_\infty
    &=
    \tfrac1n \normin{X^\top(y - X\betahat -\varepsilon)}_\infty \nonumber \\
    & \leq
    \tfrac1n \normin{X^\top(y - X\betahat)}_\infty
    + \tfrac1n \normin{X^\top \varepsilon}_\infty \nonumber \\
    & \leq
    \lambda (1 + \eta)\frac{\norm{\varepsilon}_2}{\sqrt{n}}
    + \tfrac1n \normin{X^\top \varepsilon}_\infty \nonumber \\
    & \leq
    \lambda (1 + \eta)\frac{\norm{\varepsilon}_2}{\sqrt{n}}
    +     \lambda (1 - \eta)\frac{\norm{\varepsilon}_2}{\sqrt{n}} \nonumber \\
    & \leq
    2 \lambda \frac{\norm{\varepsilon}_2}{\sqrt{n}} \nonumber \\
    & \leq
    2 \lambda \sigmamax
  \end{align}
  %
For \Cref{lem:smth_sqrt_lso_bds_pred_b}, the Smoothed \sqrtlfull fits the \cref{pb:generic_optim_pb} with $f = \frac{1}{\sqrt{n}} \normin{\cdot} \square \omega_{\sigmamin} $. \mm{isn't the sqrt n inside the argument?}
  On $ \left \{ \norm{\varepsilon}_2 / \sqrt{n} \geq \sigma_0  \geq \sigmamin \right \} \supset \cA_1$, $\partial f (\varepsilon) = \left\{ \frac{\varepsilon}{\sqrt{n} \norm{\varepsilon}} \right\}$.
  Moreover since we are on $\cA_1$ we have:
  \begin{equation}
    \left\{
      \frac{\norm{X^\top \varepsilon}_\infty}
      {\sqrt{n} \norm{\varepsilon}_2 }
      \leq
      (1 - \eta) \lambda
    \right\} \enspace, \text{ with } \frac{\varepsilon}
    {\sqrt{n} \norm{\varepsilon}_2 }  \in \partial f (\varepsilon) \nonumber \enspace .
  \end{equation}
 This allows us to apply \Cref{lem:bds_S_c_S} with $c_3 = 1 - \eta$, leading to the desired result.
  % \begin{align}
  %   \cA_1 \eqdef
  %   \left\{
  %     \frac{\norm{X^\top \varepsilon}_\infty}
  %     {\sqrt{n} \norm{\varepsilon}_2 }
  %     \leq
  %     (1 - \eta) \lambda
  %   \right\}
  %   \cap
  %   \{ \sigmamax \geq \norm{\varepsilon}_2 / \sqrt{n} \geq \sigma_0 \}
  % \end{align}
%
  % As before the proof of \Cref{lem:smth_sqrt_lso_bds_pred_b} comes from the minimality of $\betahat$:
  % \begin{align}
  %   \norm{\cdot}_2 \infconv \omega_{\sigmamin} \left( \frac{1}{\sqrt{n}}  \hat \varepsilon  \right )
  %   + \lambda \normin{\betahat}_1
  %   & \leq
  %   \norm{\cdot}_2 \infconv \omega_{\sigmamin} \left( \frac{1}{\sqrt{n}}  \varepsilon \right )
  %   + \lambda \normin{\betastar}_1 \nonumber \\
  %   \frac{1}{\sqrt{n}} \normin{\hat \varepsilon}_2
  %   + \lambda \normin{\betahat}_1
  %   & \leq
  %   \norm{\cdot}_2 \infconv \omega_{\sigmamin} \left( \frac{1}{\sqrt{n}}  \varepsilon \right )
  %   + \lambda \normin{\betastar}_1 \nonumber \\
  %   & \leq
  %   \frac{1}{\sqrt{n}} \normin{\varepsilon}_2
  %   + \lambda \normin{\betastar}_1 & \text{which leads to} \nonumber \\
  %   \frac{1}{\sqrt{n}} \normin{\hat \varepsilon}_2 -  \frac{1}{\sqrt{n}} \normin{\varepsilon}_2
  %   &\leq  \lambda \normin{\betastar}_1 -  \lambda \normin{\hat \beta}_1
  %   \enspace .
  %   \label{eq:smoothed_sqrtlasso_minimality}
  % \end{align}
  % %
  % Let us bound the right hand side of \Cref{eq:smoothed_sqrtlasso_minimality}:
  % \begin{align}
  %   \normin{\betastar}_1 - \normin{\betahat}_1
  %   &=
  %   \normin{\betastar_S}_1
  %   - \normin{\betahat_S}_1 - \normin{\betahat_{S^c}}_1 \nonumber\\
  %   %
  %   &=
  %   \normin{\betastar_S}_1
  %   - \normin{\betahat_S}_1
  %   - \normin{(\betastar - \betahat)_{S^c}}_1 \nonumber\\
  %   &\leq
  %   %
  %   \normin{(\betastar - \betahat)_S}_1
  %   - \normin{(\betastar - \betahat)_{S^c}}_1
  %   = \normin{\Delta_S}_1
  %   - \normin{\Delta_{S^c}}_1
  %   \enspace . \label{eq:smoothed_sqrtlasso_upper_bound}
  % \end{align}
  % %
  % Let us bound the left hand side of \Cref{eq:smoothed_sqrtlasso_minimality}.
  % Let $h : \beta \mapsto \norm{y - X \beta }_2$.
  % By convexity of $h$:\mm{reread with Quentin}
  % \begin{align}
  %   \normin{y - X \betahat}_2
  %   -  \normin{y - X \betastar}_2
  %   &\geq
  %   \left \langle
  %       z, \betahat - \betastar
  %   \right \rangle \quad, \quad z \in \partial h(\betastar)
  %   \enspace .
  % \end{align}
  % On the set $ \{ \beta: \norm{y - X \beta}_2 / \sqrt{n} \geq \sigmamin \}$,
  % % $h (\beta) = \frac{1}{\sqrt{n}}  \normin{y - X \beta}_2 $
  % and $\partial h (\beta^*) = \left \{ \frac{X^\top  (y - X \beta)}{ \normin{y - X \beta}_2} \right \}$.
  % %
  % On the event $\{ \norm{\varepsilon}_2 / \sqrt{n} \geq \sigma_0 \geq \sigmamin \}$ this leads to
  % \begin{align}
  %   \normin{\hat \varepsilon}_2
  %   -  \normin{\varepsilon}_2
  %   &\geq
  %   \left \langle
  %     \frac{X^\top\varepsilon}{\norm{\varepsilon}_2},
  %     \Delta
  %   \right \rangle \nonumber\\
  %   %
  %   &\geq
  %   - \frac{\norm{X^\top\varepsilon}_\infty \norm{\Delta}_1}{ \norm{\varepsilon}_2} & \text{(using H\"older inequality)} \nonumber\\
  %   %
  %   &\geq
  %   - (1-\eta) \lambda \sqrt{n} \norm{\Delta}_1 & \text{on}
  %   \left\{
  %       \frac{\norm{X^\top \varepsilon}_\infty}
  %       {\sqrt{n} \norm{\varepsilon}_2 }
  %       \leq
  %       (1 - \eta) \lambda\right\} \supset \cA_1
  %   \enspace , \label{eq:smoothed_sqrtlasso_lower_bound}
  %   % \enspace .
  % \end{align}
  % %
  % Combining \Cref{eq:smoothed_sqrtlasso_minimality,eq:smoothed_sqrtlasso_upper_bound,eq:smoothed_sqrtlasso_lower_bound} leads to:
  % \begin{align}
  %   - (1-\eta)
  %   \left (
  %     \normin{\Delta_S}_1
  %     + \normin{\Delta_{S^c}}_1
  %   \right )
  %   = - (1-\eta) \norm{\Delta}_1
  %   &\leq
  %   \normin{\Delta_S}_1 - \normin{\Delta_{S^c}}_1 & \text{and thus}
  %   \enspace, \\
  % % \end{align}
  % % %
  % % and thus
  % % %
  % % \begin{align}
  %   \norm{\Delta_{S^c}}_1
  %   &\leq
  %   \left (\frac{2}{\eta} - 1 \right) \norm{\Delta_S}_1
  %   \enspace .
  % \end{align}
  %
\end{proof}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bounds in estimation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The proof is the same that for the \sqrtlfull.


==> sections/app_sqrtlasso.tex <==
%!TEX root = ../bounds.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Bounds for the Square Root Lasso}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we derive bounds for the \sqrtlfull.
%
% \jo{same question about exponent $\delta$ in the $\betahat$ notation}
% \qbe{I guess you meant $\lambda$. Neither vdG or Karim Lounici put $\lambda$ in exponent, maybe we could stick to their notation for the moment}
% \mm{I prefer lighter notation too, $\lambda$ does not vary so I would not put it as a dependency}
\begin{definition}[\sqrtlfull]
  The \sqrtlfull estimator is defined as the solution of the optimization problem:
    \begin{problem}\label{pb:sqrt}
      \betahat
      \eqdef
      \argmin_{\beta \in \bbR^p}
      \frac{1}{\sqrt{n}} \normin{y-X \beta}_{2}
      +\lambda \normin{\beta}_{1}
      \enspace .
  \end{problem}
\end{definition}
%
\begin{restatable}[Bounds in prediction]{theorem}{restatesqrtlassosupnorm}
  \label{thm:sqrtlasso_sup_norm}
  Take $\lambda = A \sqrt{(\log p) / n}$ and $A > 2 \sqrt{2}$.
  %
  Let $\lambda$, $\eta$, and $\sigma_0$ verify \Cref{assum:high_noise}.
  Let \Cref{assum:gauss_noise,assum:mut_inco} be satisfied, then
  \begin{align}
  \bbP \left(\normin{\betahat-\betastar}_\infty  \leq c_2 \lambda \sigmamax \right)
    \geq
  1 - \quentin{to compute} - (1 + e^2) e^{-n / 24}\enspace,
   \end{align}
   with
   $c_2 = \frac{3}{2}
      \left
          (1 + \frac{16}{7(\alpha - 1)}
      \right )$, $c_0= \frac{2}{\eta} - 1$, $\alpha$ satisfying \Cref{assum:mut_inco} and $\eta$ satisfying \Cref{assum:high_noise}.
\end{restatable}\mm{TODO this must not appear in appendix}
The proof, inspired from the Lasso case, again relies on technical results detailed in \Cref{sub:kkt_sqrt,sub:dantzig_sqrt}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Optimality conditions}
\label{sub:kkt_sqrt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% A Lagrangian for \Cref{pb:sqrt} is, for $\beta \in \bbR^p, \theta \in \bbR^n, z \in \bbR^n$,
% \begin{align}
%   \cL(\beta, \theta, z)
%   = \frac{1}{\sqrt{n}} \norm{z}_{2}
%     + \lambda \normin{\betahat}_{1}
%     + \lambda \theta^\top (z - y + X  \beta ) \enspace,
% \end{align}
% %
% The KKT conditions reads:
% \begin{align}
%   \begin{cases}
%     \nabla_\theta \cL(\hat \beta, \hat \theta, \hat z) = 0 \enspace, \\
%     0 \in \partial_\beta \cL(\hat \beta, \hat \theta, \hat z) \enspace,\\
%     0 \in \partial_z \cL(\hat \beta, \hat \theta, \hat z) \enspace,
%   \end{cases}
% i.e., \quad
% \begin{cases}
%   \hat z
%   = y - X \hat\beta \enspace, \\
%   - X^\top \hat \theta
%   \in \partial \normin{\cdot}_1 (\hat \beta) \enspace,\\
%   \lambda \sqrt{n} \hat \theta
%   \in \partial \normin{\cdot}_2 (y - X \hat \beta) \enspace, \label{eq:third_opt_cond_conco}
% \end{cases}
% \end{align}
% with
% \begin{equation}
%   \partial \normin{\cdot}_2(x) =
%   \begin{cases}
%     \frac{x}{\norm{x}_2}  &\text{, if } x \neq 0 \enspace, \\
%     \condsetin{z \in \bbR^{n}}{\norm{z}_2 \leq 1 } &\text{else} \enspace ,
%   \end{cases}
% \end{equation}
% %
% and
% %
% \begin{equation}
%   \partial \normin{\cdot}_1(x) =
%   \condsetin{z}{z_i = \sign(x_i) \text{ if } x_i \neq 0, z_i \in [-1, 1] \text{ else}} \enspace .
% \end{equation}
% %
% Additionally,
% %
% \begin{align}
%   \min_{\beta, z} \cL(\beta, \theta, z)
%       &=
%       - \lambda \theta^\top y
%       + \min_\beta \left(
%             \lambda \norm{\beta}_1
%             + \lambda \theta^\top  X \beta
%           \right)
%       + \min_z \tfrac{1}{\sqrt{n}} \left(
%         \norm{z}_2
%         + \lambda \sqrt{n} \theta^\top z
%         \right)
%         \nonumber\\
%       &=
%       - \lambda \theta^\top y
%       - \lambda \max_\beta \left(
%           - \theta^\top X \beta
%           - \normin{\beta}_1
%         \right)
%       - \tfrac{1}{\sqrt{n}} \max_z  \left(
%             \lambda \sqrt{n} \theta^\top z
%             - \norm{z}_2
%           \right)
%           \nonumber\\
%       &=
%       - \lambda \theta^\top y
%       -  \iota_{\cB_\infty}(X^\top \theta )
%       -  \iota_{\cB_2}(\lambda\sqrt{n} \theta)
%       \nonumber \enspace.
% \end{align}
%
% Therefore a dual formulation $\max_{\theta} \min_{\beta, z} \cL(\beta, \theta, z) $ of \Cref{pb:sqrt} is:
The square-root Lasso fits \Cref{pb:generic_optim_pb} with $f = \tfrac{1}{\sqrt{n}} \normin{\cdot}_2$.
\Cref{pb:dual_generic} instantiates as:
\begin{problem}\label{pb:dual_sqrt}
  \hat \theta \in \argmax_{\theta \in \bbR^n}  \lambda \theta^\top y
      \quad \st \quad \normin{X^\top \theta}_\infty \leq 1 \quad \text{and} \quad
    \normin{\theta }_2 \leq 1 / \lambda \sqrt{n}
    \enspace ,
\end{problem}
and the Kuhn-Tucker conditions as
\begin{equation}
  \begin{cases}
    \hat z
    - X^\top \hat \theta
    \in \partial \normin{\cdot}_1 (\hat \beta) \enspace,\\
    \lambda \sqrt{n} \hat \theta
    \in \partial \normin{\cdot}_2 (y - X \hat \beta) \enspace, \label{eq:third_opt_cond_conco}
  \end{cases}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Dantzig constraint set}
\label{sub:dantzig_sqrt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The goal of this subsection is to show an inequality similar to the Dantzig constraint set for the \sqrtlfull.
Let $\hat \epsilon = y - X \betahat$, if $\hat \epsilon \neq 0$, the optimality conditions \Cref{eq:third_opt_cond_conco} lead to:
\begin{align}
  \thetahat
  & = \frac{1}{\lambda \sqrt{n}} \frac{\hat \epsilon}{\normin{\hat \epsilon}_2} \enspace , \nonumber\\
  %
  X^{\top} \thetahat
  & =  \frac{1}{\lambda\sqrt{n}} \frac{X^{\top} \hat \epsilon}{\normin{\hat \epsilon}_2} \enspace , \nonumber\\
  %
  1
  & \geq \frac{1}{\lambda\sqrt{n}}
  \frac{\normin{X^{\top}\hat \epsilon}_\infty }{\normin{\hat \epsilon}_2} \nonumber
  \enspace .
\end{align}
%
This shows that the \sqrtlfull satisfies a modified Dantzig constraint:
%
\begin{align}\label{eq:dantzig_constr_sqrtl_sigmahat}
  \frac{1}{n} \norm{ X^{\top} \hat \varepsilon}_\infty
  \leq
  \lambda \sigmahat
  \enspace ,
  \text{ with } \sigmahat \eqdef  \frac{1}{\sqrt{n}}\normin{\hat \varepsilon}_2, \text{ and } \hat \epsilon = y - X \hat \beta \enspace .
\end{align}
Note that the previous constraint is also satisfied when $\hat \epsilon =  0$.

% Since $\sigmahat$ depends on $\betahat$, \Cref{eq:dantzig_constr_sqrtl_sigmahat} is not  a satisfying bound.
% However, under additional assumptions, %-- roughly, that the noise is sufficiently uncorrelated with the columns of $X$, but high enough to be estimated --
% it can be shown that $\sigmahat$ is close to $\sigma$:
% %
% \begin{lemma}[{\citet[Lemma 3.1 p.29]{vandeGeer16}}]\label{lem:approx_sigma}
%   If \Cref{assum:high_noise} is satisfied, then on the event
%   \begin{align}
%     % \cA_1 \eqdef
%     \left\{
%       \norm{X^\top \varepsilon}_\infty
%        \leq (1 - \eta) \lambda  {\sqrt{n} \norm{\varepsilon}_2 } \right\}
%     \cap
%     \{ \norm{\varepsilon}_2  \sqrt{n} \geq \sigma_0 \}
%     \supset \cA_1 \enspace ,
%   \end{align}
%  we have:
%   \begin{align}
%     \left | \frac{\norm{\hat \varepsilon}_2}{\norm{ \varepsilon }_2 } - 1 \right |
%     \leq \eta \enspace .
%   \end{align}
% \end{lemma}
% %
% \quentin{The more I think about it the more it looks like we do not need this $\sigma_0$}
%
% \qbe{It turns out that we do not need the full lemma of vdG, since we only need the UPPER bound on $ \hat  \varepsilon$ we could softness the hypothesis, wdyt ?}
%
\begin{lemma}
  Suppose that \Cref{assum:high_noise} is satisfied, then:
  \begin{equation}
    \frac{\norm{\varepsilon}_2}{\sqrt{n}} \leq (1 + \eta) \sigmamax
  \end{equation}
\end{lemma}
%
\begin{proof}
  The proof comes for the minimality of the estimator:
  \begin{align}
    \frac{1}{\sqrt{n}} \normin{\hat \epsilon}_{2} + \lambda \normin{\hat \beta}_{1}
    &\leq \frac{1}{\sqrt{n}} \normin{\epsilon}_{2} + \lambda \normin{\beta^*}_{1} \nonumber\\
    \frac{1}{\sqrt{n}} \normin{\hat \epsilon}_{2}
    & \leq  \frac{1}{\sqrt{n}} \normin{\epsilon}_{2} + \lambda \normin{\beta^*}_{1} \nonumber\\
    & \leq  \sigmamax + \lambda \normin{\beta^*}_{1} & \text{using $\frac{1}{\sqrt{n}} \normin{\epsilon}_{2} \leq \sigmamax$}\nonumber\\
    & \leq  ( 1 + \eta )\sigmamax
  \end{align}
\end{proof}
%
Combining \Cref{eq:dantzig_constr_sqrtl_sigmahat,assum:high_noise} leads to the following result: on $\cA_1$,
\begin{align}\label{eq:dantzig_constr_sqrtl_sigma}
  \frac{1}{n} \norm{ X^{\top} \hat \varepsilon}_\infty
  \leq
  \lambda (1 + \eta) \frac{\norm{\varepsilon}_2}{\sqrt{n}}
  \enspace .
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bounds in prediction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Let $\cA_1$ be the following event: \mathurin{$\cA_1$ was defined to be something else in the lines above}
\begin{align}
  \cA_1 \eqdef
  \left\{
    \frac{\norm{X^\top \varepsilon}_\infty}
    {\sqrt{n} \norm{\varepsilon}_2 }
    \leq
    (1 - \eta) \lambda
  \right\}
  \cap
  \{ \sigmamax \geq \norm{\varepsilon}_2 / \sqrt{n} \geq \sigma_0 \}
\end{align}
%
\begin{lemma}\label{lem:sqrtlasso_bds_pred}
  Let $\lambda$ $\eta$, and $\sigma_0$ verify \Cref{assum:high_noise}.
  Let \Cref{assum:gauss_noise,assum:mut_inco} be satisfied.
  With $\Delta = \betahat - \betastar$, $c_0=\frac{2}{\eta} - 1$, $0 \leq \eta \leq 1$, on $\cA_1$:
  \begin{lemmaenum}
      \item
          $\tfrac1n \normin{X^\top(X\betastar - X\betahat)}_\infty
          \leq
          2 \sigmamax  \lambda
          % \frac{\norm{\varepsilon}_2}{\sqrt{n}}
          $
          \enspace , \label{lem:sqrtlso_bds_pred_a}
      \item $\norm{\Delta_{S^{* c}}}_{1}
            \leq
            c_0 \norm{\Delta_{S^*}}_{1}
            \enspace .$
            \label{lem:sqrtlso_bds_pred_b}
  \end{lemmaenum}
\end{lemma}
%
\begin{proof}
  As for the Lasso (\Cref{lem:lso_bds_pred}), the proof of \Cref{lem:sqrtlso_bds_pred_a} comes from the KKT conditions and the concentration on $\cA_1$:
  \begin{align}
    \tfrac1n \normin{X^\top(X\betastar - X\betahat)}_\infty
    &=
    \tfrac1n \normin{X^\top(y - X\betahat -\varepsilon)}_\infty \nonumber \\
    & \leq
    \tfrac1n \normin{X^\top(y - X\betahat)}_\infty
    + \tfrac1n \normin{X^\top \varepsilon}_\infty
    & \text{(using triangle inequality)} \nonumber \\
    & \leq
    \lambda (1 + \eta)\frac{\norm{\varepsilon}_2}{\sqrt{n}}
    + \tfrac1n \normin{X^\top \varepsilon}_\infty
    & \text{(using \Cref{eq:dantzig_constr_sqrtl_sigmahat})} \nonumber \\
    & \leq
    \lambda (1 + \eta)\frac{\norm{\varepsilon}_2}{\sqrt{n}}
    +     \lambda (1 - \eta)\frac{\norm{\varepsilon}_2}{\sqrt{n}} & \text{(using $\left\{
      \frac{\norm{X^\top \varepsilon}_\infty}
      {\sqrt{n} \norm{\varepsilon}_2 }
      \leq
      (1 - \eta) \lambda
    \right\} \supset \cA_1$)}  \nonumber\\
    & \leq
    2 \lambda \frac{\norm{\varepsilon}_2}{\sqrt{n}} \nonumber\\
  & \leq
  2 \lambda \sigmamax & \text{(using $\left \{ \sigmamax \geq \frac{\norm{\varepsilon}_2}{\sqrt{n}} \right \} \supset \cA_1$).} \nonumber
\end{align}
%
To prove \Cref{lem:sqrtlso_bds_pred_b}, the \sqrtlfull fits the \cref{pb:generic_optim_pb} with $f = \frac{1}{\sqrt{n}} \normin{\cdot}$.
  On $ \left \{ \norm{\varepsilon}_2 / \sqrt{n} \geq \sigma_0  \geq \sigmamin \right \} \supset \cA_1$, $\partial f (\varepsilon) = \left\{ \frac{\varepsilon}{\sqrt{n} \norm{\varepsilon}} \right\}$.
  Moreover since we are on $\cA_1$ we have:
  \begin{equation}
    \left\{
      \frac{\norm{X^\top \varepsilon}_\infty}
      {\sqrt{n} \norm{\varepsilon}_2 }
      \leq
      (1 - \eta) \lambda
    \right\} \enspace, \text{ with } \frac{\varepsilon}
    {\sqrt{n} \norm{\varepsilon}_2 }  \in \partial f (\varepsilon) \nonumber \enspace .
  \end{equation}
 This allows us to apply \Cref{lem:bds_S_c_S} with $c_3 = 1 - \eta$, leading to the desired result.
%
% For \Cref{lem:sqrtlso_bds_pred_b}, we again use the minimality of $\betahat$:
%   \begin{align}
%     \frac{1}{\sqrt{n}} \normin{y - X \betahat}_2
%     + \lambda \normin{\betahat}_1
%     & \leq
%     \frac{1}{\sqrt{n}} \normin{y - X \betastar}_2
%     + \lambda \normin{\betastar}_1  \nonumber \\
%     %
%     \frac{1}{\sqrt{n}} \normin{y - X \betahat}_2
%     - \frac{1}{\sqrt{n}} \normin{y - X \betastar}_2
%     & \leq
%      \lambda \normin{\betastar}_1
%     - \lambda \normin{\betahat}_1 \enspace .
%     \label{eq:sqrtlasso_minimality}
%   \end{align}
% %
%   Let us bound the right hand side of \Cref{eq:sqrtlasso_minimality}:
%   \begin{align}
%     \normin{\betastar}_1 - \normin{\betahat}_1
%     &=
%     \normin{\betastar_{S^*}}_1
%     - \normin{\betahat_{S^*}}_1 - \normin{\betahat_{{S^{*c}}}}_1 \nonumber & \text{(using $\normin{\betahat}_1 =  \normin{\betahat_{S^*}}_1 + \normin{\betahat_{S^{*c}}}_1 $)}\\
%     %
%     &=
%     \normin{\betastar_{S^*}}_1
%     - \normin{\betahat_{S^*}}_1
%     - \normin{(\betastar - \betahat)_{{S^{*c}}}}_1  & \text{(using $\betastar_{{S^{*c}}} = 0$)}
%     \nonumber \\
%     &\leq
%     %
%     \normin{(\betastar - \betahat)_{S^*}}_1
%     - \normin{(\betastar - \betahat)_{S^{*c}}}_1 & \text{ (using triangle inequality)} \nonumber \\
%     %
%     & \leq \normin{\Delta_{S^*}}_1
%     - \normin{\Delta_{S^{*c}}}_1
%     \enspace . \label{eq:sqrtlasso_upper_bound}
%   \end{align}
%   %
%   Let us bound the left hand side of \Cref{eq:sqrtlasso_minimality}.
%   With probability 1, $y - X \betastar = \varepsilon \neq 0$, thus convexity of $\beta \mapsto \normin{ y - X \beta}_2$ leads to:
%   \begin{align}
%     \normin{y - X \betahat}_2
%     -  \normin{y - X \betastar}_2
%     &\geq
%     \left \langle
%       \frac{X^\top (y - X \betastar)}{\normin{y - X \betastar}_2},
%       \betahat - \betastar
%     \right \rangle
%     \enspace \nonumber\\
%     %
%     &\geq
%     \left \langle
%       \frac{X^\top\varepsilon}{\norm{\varepsilon}_2},
%       \Delta
%     \right \rangle \nonumber \\
%     &\geq
%     - \frac{\norm{X^\top\varepsilon}_\infty \norm{\Delta}_1}{ \norm{\varepsilon}_2} & \text{(Using H\"older inequality)}
%     \nonumber\\
%     &\geq
%     - (1-\eta) \lambda \sqrt{n} \norm{\Delta}_1
%     & \text{(using
%         $\left\{
%           \frac{\norm{X^\top \varepsilon}_\infty}
%           {\sqrt{n} \norm{\varepsilon}_2 }
%           \leq
%           (1 - \eta) \lambda\right\}
%           \supset \cA_1$
%       )}
%     \enspace . \label{eq:sqrtlasso_lower_bound}
%   \end{align}
%   %
%   Combining \Cref{eq:sqrtlasso_minimality,eq:sqrtlasso_upper_bound,eq:sqrtlasso_lower_bound} leads to:
%   \begin{align}
%     - (1-\eta) \norm{\Delta}_1
%     &\leq
%     \normin{\Delta_{S^*}}_1 - \normin{\Delta_{S^{*c}}}_1
%   \nonumber\\
%   - (1-\eta) \Big ( \normin{\Delta_{S^*}}_1
%           + \normin{\Delta_{S^{*c}}}_1 \Big )
%   & \leq
%   \normin{\Delta_{S^*}}_1 - \normin{\Delta_{S^{*c}}}_1 & \text{leading to}\nonumber\\
%     \norm{\Delta_{S^{*c}}}_1
%     &\leq
%     \left (\frac{2}{\eta} - 1 \right) \norm{\Delta_{S^*}}_1
%     \enspace .
%   \end{align}
  %
\end{proof}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Control of the event}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{lemma}[Bound on $\cA_1$]
  \label{lem:bounds_on_event_sqrtlasso}
  \begin{align}
    \bbP(\cA_1)
    \geq
      1 - p^{1 - A^2 / 8}
      - \Phi_n(\frac{\sigma_0}{\sigma}, \frac{\sigmamax}{\sigma})
    \enspace,
  \end{align}
  with \quentin{TODO compute A exactly} with $\Phi_n(\cdot, \cdot)$ the repartition function of a chi-square random variable with $n$ degrees of freedom:
   $\Phi_n(a, b) = \bbP \left(
   a \leq  \frac{\norm{\varepsilon}_2}{\sigma \sqrt{n}}  \leq b
   \right ) $.
   Moreover if $\sigma_0 = \sigma / \sqrt{2}$ and $\sigmamax = 2 \sigma$:
   \begin{align}
    \bbP(\cA_1)
    \geq
      1 - p^{1 - A^2 / 8}
      - (1 + e^2)e^{- n / 24}
      \enspace, \nonumber
  \end{align}
  \end{lemma}
%
\Cref{lem:bounds_on_event_sqrtlasso} shows that values of $\sigma_0$ (\resp $\sigmamax$) does not need to be unrealistically small (\resp unrealistically high) for the probability to be very high.
%
\begin{proof}
  \begin{align}
    \bbP(\cA_1)
      % &= 1 - \bbP(\cA_1^c)\\
      &= 1 - \bbP \left( \left \{
        \frac{\norm{X^\top \varepsilon}_\infty}
        {\sqrt{n} \norm{\varepsilon}_2 }
        \leq
        (1 - \eta) \lambda
      \right \}^c
        \cup
        \left\{
          \sigmamax \geq \norm{\varepsilon}_2 / \sqrt{n} \geq \sigma_0
        \right \}^c
        \right) \nonumber \\
      %
      & \geq 1 - \bbP \left(
        \frac{\norm{X^\top \varepsilon}_\infty}
        {\sqrt{n} \norm{\varepsilon}_2 }
        \geq
        (1 - \eta) \lambda
     \right)
        - \bbP \left ( \{ \sigmamax \geq \norm{\varepsilon}_2 / \sqrt{n} \geq \sigma_0 \}^c \right) \nonumber
  \end{align}
\end{proof}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bounds in estimation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\restatesqrtlassosupnorm*

\begin{proof}
  Let us warn the reader that in the following proof the results are considered on the event $\cA_1$.
  Let $\Psi$ and $\alpha$ satisfy \Cref{assum:mut_inco}, \Cref{lem:sqrtlso_bds_pred_b,lem:bnd_l_infty_l_infty} leads to:
  \begin{align}
    \normin{\Delta}_\infty
    & \leq \left(
        1 + \frac{16}{7(\alpha - 1) } \right) \norm{\Psi \Delta}_\infty \nonumber \\
    & \leq \frac{3}{2}\left(
        1 + \frac{16}{7(\alpha - 1) } \right) \lambda \sigmamin & \text{(using \Cref{lem:sqrtlso_bds_pred_a}).} \nonumber
  \end{align}
  Combined with \Cref{lem:bounds_on_event_sqrtlasso} this lead to the desired results.
\end{proof}

